Consensus, dissensus and synergy between clinicians and specialist foundation models in radiology report generation

Radiology reports are an instrumental part of modern medicine, informing key clinical decisions such as diagnosis and treatment. The worldwide shortage of radiologists, however, restricts access to expert care and imposes heavy workloads, contributing to avoidable errors and delays in report delivery. While recent progress in automated report generation with vision-language models offer clear potential in ameliorating the situation, the path to real-world adoption has been stymied by the challenge of evaluating the clinical quality of AI-generated reports. In this study, we build a state-of-the-art report generation system for chest radiographs, $\textit{Flamingo-CXR}$, by fine-tuning a well-known vision-language foundation model on radiology data. To evaluate the quality of the AI-generated reports, a group of 16 certified radiologists provide detailed evaluations of AI-generated and human written reports for chest X-rays from an intensive care setting in the United States and an inpatient setting in India. At least one radiologist (out of two per case) preferred the AI report to the ground truth report in over 60$\%$ of cases for both datasets. Amongst the subset of AI-generated reports that contain errors, the most frequently cited reasons were related to the location and finding, whereas for human written reports, most mistakes were related to severity and finding. This disparity suggested potential complementarity between our AI system and human experts, prompting us to develop an assistive scenario in which Flamingo-CXR generates a first-draft report, which is subsequently revised by a clinician. This is the first demonstration of clinician-AI collaboration for report writing, and the resultant reports are assessed to be equivalent or preferred by at least one radiologist to reports written by experts alone in 80$\%$ of in-patient cases and 60$\%$ of intensive care cases.

==> figures/table1.tex <==
\begin{table}[ht]
    \centering
    \caption{Report generation accuracy on MIMIC-CXR. note that the numbers are besed on reported numbers.}
    \label{tab:table_mimic}
    \footnotesize
    \begin{tabular}{|*{7}{c|}}
        \hhline{~*{6}{-}}
        % \hline
        \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{NLG Metrics}} &\multicolumn{3}{c|}{\textbf{Clinical Metrics}}  \\\hline
        % \multicolumn{1}{c|}{} & A & B & C & D & E & F \\ \hline
        \textbf{Model} & \textbf{CIDEr} & \textbf{BLEU4} & \textbf{Rouge-L}  & \textbf{CheXpert-F1-all} & \textbf{CheXpert-F1-top5} & \textbf{Radgraph}\\ \hline
        % use \gradient{} in the cells with a value between \minval and \maxval!
        Mini-Flamingo (Ours) & \gradient{0.138} & \gradient{0.101} & \gradient{0.297} & \gradient{0.519} & \gradient{0.580} & \gradient{0.205}   \\ \hline
        Med-PaLM-M, 12B \citep{tu2023generalist}& \gradient{0.234} & \gradient{0.104} & \gradient{0.262} & \gradient{0.514} & \gradient{0.565} & \gradient{0.252}   \\ \hline
        $\mathcal{M}^2$ Transformer \citep{miura2021} & \gradient{0.509} & \gradient{0.114} &  \gradient{-} & \gradient{-} & \gradient{0.567} & \gradient{0.110}   \\ \hline
        R2Gen \citep{chen2020} & \gradient{-} & \gradient{0.103} & \gradient{0.277} & \gradient{0.228} & \gradient{0.346} & \gradient{0.057}   \\ \hline
        R2GenGPT \citep{wang2023r2gengpt} & \gradient{0.269} & \gradient{0.134} & \gradient{0.297} & \gradient{0.389} & \gradient{-} & \gradient{-}   \\ \hline
        CXR-RePaiR \citep{Krishnan2021} & \gradient{-} & \gradient{0.021} & \gradient{0.143} & \gradient{0.281} & \gradient{-} & \gradient{0.091}   \\ \hline
        CvT-21DistillGPT2 \citep{NICOLSON2023} & \gradient{0.361} & \gradient{0.124} & \gradient{0.285} & \gradient{0.384} & \gradient{-} & \gradient{0.073}   \\ \hline
         RGRG \citep{tanida2023interactive} & \gradient{0.495} & \gradient{0.126} & \gradient{0.264} & \gradient{0.447} & \gradient{0.547} & \gradient{-}   \\ \hline
         BioVil-T \citep{bannur2023learning} & \gradient{-} & \gradient{0.092} & \gradient{0.296} & \gradient{0.317} & \gradient{-} & \gradient{-}   \\ \hline
         METransformer \citep{wang2023metransformer}  & \gradient{0.362} & \gradient{0.124} & \gradient{0.291} & \gradient{0.311} & \gradient{-} & \gradient{-}   \\ \hline
    \end{tabular}
\end{table}

